NNLL resummation for squark-antisquark production

We report on the resummation of soft-gluon emissions for squark-antisquark production at next-to-next-to-leading-logarithmic (NNLL) accuracy. We will put particular emphasis on the one loop hard matching coefficients required to perform the resummation. Furthermore we will discuss the numerical effect of the different ingredients in the corrections. We find a significant reduction in the scale uncertainty and a considerable increase in the prediction of the total cross section at the central scale. Compared to the next-to-leading order prediction, the corrections increase the cross section by up to 30% for 1.5 TeV squarks at a centre-of-mass energy of 7 TeV at the LHC.

==> preprint.tex <==
DESY 11-254

